Statistical Properties of the Probabilistic Numeric Linear Solver BayesCG

We analyse the calibration of BayesCG under the Krylov prior, a probabilistic numeric extension of the Conjugate Gradient (CG) method for solving systems of linear equations with symmetric positive definite coefficient matrix. Calibration refers to the statistical quality of the posterior covariances produced by a solver. Since BayesCG is not calibrated in the strict existing notion, we propose instead two test statistics that are necessary but not sufficient for calibration: the Z-statistic and the new S-statistic. We show analytically and experimentally that under low-rank approximate Krylov posteriors, BayesCG exhibits desirable properties of a calibrated solver, is only slightly optimistic, and is computationally competitive with CG.

==> UQMisc.tex <==
\subsubsection{\textcolor{red}{Hierarchical BayesCG, Will probably not include}}

\textcolor{red}{I probably will not include this section. The hierarchical scale is somewhat complicated to explain and I do not use it in the rest of the paper. The error estimate scale in \cite{BCG:Supp} uses the chi-square $Z$-statistic instead of the F $Z$-statistic. If this is not a mistake, motivating the Krylov prior (which has a scale built into it) with the error estimate scale is probably good enough.}

The covariance scale is computed in a hierarchical Bayesian procedure and causes the BayesCG posterior to be a multivariate T distribution \cite[Proposition 11]{Cockayne:BCG}.

We present the hierarchical BayesCG posterior from \cite[Proposition 11]{Cockayne:BCG} after defining the multivariate T distribution.
\begin{definition}{\textcolor{red}{Got from wikipedia. Find better source}}
  \label{Def:MVT}
  The multivariate T distribution with mean $\xvec$, matrix parameter $\Sigmat$, and $p$ degrees of freedom is the distribution of
  \begin{equation*}
    \frac{\Xrv}{\sqrt{\Yrv/p}}-\xvec \sim MVT_p(\xvec,\Sigmat),
  \end{equation*}
  where $\Xrv\sim\N(\xvec,\Sigmat)$ is a Gaussian random variable and $\Yrv\sim\chi^2_p$ is a chi-square distributed random variable.
\end{definition}

\begin{theorem}{{\cite[Proposition 11]{Cockayne:BCG}}}
  \label{T:ScaledBayesCG}
  If $\mu_m = \N(\xvec_m,\Sigmat_m)$ is the BayesCG posterior from \tref{T:XmSigmTheory}, then the BayesCG posterior distribution with a covariance scale determined in a hierarchical Bayesian procedure is
  \begin{equation*}
    MVT_m(\xvec_m,h_m\Sigmat_m) \quad \text{where} \quad h_m = \|\Smat_m^T\rvec_0\|_2^2.
  \end{equation*}
\end{theorem}

The $Z$-statistic defined in \tref{T:ZStat} requires the output distribution to be Gaussian. A modification of the $Z$-statistic that relates the error to an $F$ distribution. We present a definition of the $F$ distribution then restate the the modified $Z$-statistic from \cite[Section 6.1]{Cockayne:BCG}.

\begin{definition}
  The $F$ distribution with parameters $p$ and $q$ is the distribution of
  \begin{equation*}
    \frac{\Xrv/p}{\Yrv/q}\sim F(p,q),
  \end{equation*}
  where $\Xrv\sim\chi_p^2$ and $\Yrv\sim\chi_q^2$ are chi-square distributed random variables.
\end{definition}

\begin{theorem}[{\cite[Section 6.1]{Cockayne:BCG}}]
  \label{T:ZStatModified}
  Let $\mu_m = MVT_m(\xvec_m,h_m\Sigmat_m)$ be the scaled BayesCG posterior distribution. The modified $Z$-statistic is
  \begin{equation*}
    \Zstat(\xvec_*) = \frac{1}{\rank(\Sigmat_m)} (\xvec_*-\xvec_m)^T\frac{1}{h_m}\Sigmat_m^\dagger(\xvec_*-\xvec_m).
  \end{equation*}
  If $\mu_m$ is well calibrated, then the modified $Z$-statistic is distributed according to $F(\rank(\Sigmat_m),m)$.
\end{theorem}

Assessing the scaled BayesCG posterior with the modified $Z$-statistic is performed the same way as assessing a Gaussian output distribution in \sref{S:ZDef}. The experiments with the scaled posterior in \cite[Section 6.1]{Cockayne:BCG} show that posterior is still conservative. However, a heuristically chosen scale is examined in \cite[Section S4.3]{BCG:Supp}, and it causes the posterior to be less conservative than the unscaled and hierarchical posteriors.

\section{Background Information}

\subsection{BayesCG}

% FIRST COMMENT

The posterior $\mu_m$ is the distribution of $\Xrv$ given that the random variable $\Yrv_m := \Smat_m^T\Amat\Xrv$ has the value $\Smat_m^T\Amat\xvec_*$. The posterior can be easily computed because of the following two properties of Gaussian distributions:
\begin{description}
\item[\bf Stability] Linear transformations of Gaussian random variables, such as $\Yrv$, are Gaussian \cite[Section 1.2]{Muirhead}
\item[\bf Conjugacy] Posteriors from Gaussian priors conditioned on Gaussian random variables are Gaussian \cite[Theorem 6.20]{Stuart:BayesInverse}.
\end{description}

The formula for the BayesCG posterior originally appeared as \cite[Proposition 1]{Cockayne:BCG} and was extended to allow singular prior covariances in \cite[Theorem 2.1]{RICO20}, and we restate it below.

% SECOND COMMENT


The search direction and mean vector recursions, lines \ref{A:Line:x} and \ref{A:Line:s} in \aref{A:BayesCG} respectively, are similar to the corresponding recursions in CG. If $\Sigmat_0 = \Amat^{-1}$, then the BayesCG search directions and mean vector iterates are equal to the CG search directions and solution iterates \cite[Section 2.3]{Cockayne:BCG}. Additionally, BayesCG under the Krylov prior, which we discuss in \sref{S:Krylov}, is implemented as a CG method \cite[Algorithm 3.1]{RICO20}. Further discussion of \aref{A:BayesCG} can be found in \cite[Section 5]{Cockayne:BCG} and \cite[Section 2.2]{RICO20}.

The requirement $\xvec_*-\xvec_0\in\range(\Sigmat_0)$ in \aref{A:BayesCG} ensures that the search directions satisfy $\svec_i\not\in\ker(\Sigmat_0\Amat)$ \cite[Theorem 2.5]{RICO20}. Statistically, this requirement means that $\mu_0$ must be chosen so that $\xvec_*$ is in the support of $\mu_0$, the subset of $\Rn$ where its probability density function non-zero.


The BayesCG posterior distribution is made up of two components. The first component is a projection of the Dirac distribution on $\xvec_*$ onto $\range(\Sigmat_0\Amat\Smat_m)$. The second component is a projection of the prior $\mu_m$ onto the orthogonal complement $\range(\Sigmat_0\Amat\Smat_m)^\perp$ \cite[Proposition 3]{BCG:Rejoinder} \cite[Theorem 2.7]{RICO20}. This means $m$ iterations of BayesCG eliminate the uncertainty in $m$ dimensions of the prior distribution. Consequently, $\rank(\Sigmat_m) = \rank(\Sigmat_0) - m$ because the uncertainty on $\xvec_*$, as modeled by the posterior distribution, is in a $\rank(\Sigmat_0) - m$ dimension subspace of $\Rn$. 

In the following section we discuss in detail what it means for the posterior to be well calibrated.

\subsection{Krylov Prior}


We present our version of the Krylov Prior, a choice of prior that causes BayesCG to produce a posterior the $Z$-statistic and $S$-statistic suggest is well calibrated. Our version of the Krylov prior originally appeared in \cite[Section 3]{RICO20} and is a modification of the  ``Krylov Subspace Prior'' from \cite[Section 4.1]{Cockayne:BCG}.

The Krylov prior is important because it allows BayesCG to be implemented efficiently as a CG method and can produce accurate error estimates. We restate the definition of the Krylov prior from \cite{RICO20} and its important properties in \dref{D:KrylovPrior} and \tref{T:KrylovPrior} respectively.  We then compute the error between and low rank approximate Krylov posterior \cite[Section 3.2]{RICO20} and the full rank posterior in \sref{S:KrylovApprox}. Finally, We present a statistical interpretation of the Krylov prior in \sref{S:KrylovStat}. 

The Krylov prior is defined in terms step sizes and normalized search directions in the Conjugate Gradient method (CG), \aref{A:CG}. CG is a Krylov subspace method whose solution $\xvec_m$ satisfies the optimization property
\begin{equation*}
  \xvec_m = \argmin_{\xvec\in\xvec_0+\Kcal_m(\Amat,\rvec_0)} \|\xvec_*-\xvec\|_\Amat^2,
\end{equation*}
where $\Kcal_m(\Amat,\rvec_0)$ is the $m$ dimensional Krylov space
\begin{equation*}
  \Kcal_m(\Amat,\rvec_0) = \spn\{\rvec_0,\Amat\rvec_0, \Amat^2\rvec_0,\ldots, \Amat^{m-1}\rvec_0\}.
\end{equation*}
and $\xvec_0 + \Kcal_m(\Amat,\rvec_0)$ is the $m$ dimensional \emph{shifted} Krylov space
\begin{equation*}
  \xvec_0 + \Kcal_m(\Amat,\rvec_0) = \spn\{\xvec_0 + \rvec_0,\xvec_0 + \Amat\rvec_0, \xvec_0 + \Amat^2\rvec_0,\ldots, \xvec_0 + \Amat^{m-1}\rvec_0\}.
\end{equation*}
The CG search directions $\vvec_i$, $1\leq i \leq m$ are an $\Amat$-orthogonal basis of $\Kcal_m(\Amat,\rvec_0)$ \cite[Theorem 5.1]{Hestenes}.



Denote by $1\leq \kry\leq \dm$ the dimension of the maximal Krylov space, that is the value $\kry$ such that
\begin{equation*}
\Kcal_\kry(\Amat,\rvec_0)=\Kcal_{\kry+i} (\Amat,\rvec_0), \qquad i\geq 1.
\end{equation*}
The value $\kry$ is also known as the \textit{grade} of $\rvec_0$ with respect to $\Amat$ \cite[Definition 4.2.1]{Liesen} and the \textit{invariance index} for $(\Amat, \rvec_0)$ \cite[Section 2]{Berljafa}.

Define the matrix of normalized search directions as
\begin{equation}
  \label{Eq:VFactor}
  \Vmat \equiv \begin{bmatrix} \tilde{\vvec}_1 & \tilde{\vvec}_2 & \cdots & {\vvec}_\kry \end{bmatrix} \in\R^{n\times\kry},  \quad \tilde{\vvec}_i = \frac{1}{ \sqrt{\vvec_i^T\Amat\vvec_i}}\vvec_i,  \quad 1\leq i \leq \kry.
\end{equation}
The columns of $\Vmat$ are normalized versions of the search directions computed with $m = \kry$ iterations of \aref{A:CG}. The columns of $\Vmat$  represent an $\Amat$-orthonormal basis for $\range(\Vmat)=\Kcal_\kry(\Amat,\rvec_0)$. Additionally, define the diagonal step size matrix as
\begin{equation}
  \label{Eq:PhiFactor}
  {\Phimat} = \diag\begin{pmatrix} \phi_1 &\phi_2 & \cdots & \phi_\kry\end{pmatrix}\in\R^{\kry\times \kry} \quad 
  \phi_i = \gamma_i\|\rvec_i\|_2^2, \quad \ 1\leq i \leq \kry,
\end{equation}
where $\rvec_i$ and $\gamma_i$, $1\leq i \leq \kry$, are from \aref{A:CG}. The Krylov prior is defined in terms of the factor matrices $\Vmat$ and $\Phimat$.

\begin{definition}
\label{D:KrylovPrior}
The {\rm Krylov prior} is $\eta_0 = \N(\xvec_0,\Gammat_0)$ where
\begin{equation}
\label{Eq:KrylovPrior}
\Gammat_0 \equiv \Vmat \Phimat \Vmat^T \in\Rnn,
\end{equation}
and where the factor matrices $\Vmat$ and $\Phimat$ are defined in \eref{Eq:VFactor} and \eref{Eq:PhiFactor} respectively.
\end{definition}

BayesCG with the Krylov prior produces mean vector iterates equal to the CG iterates and a posterior covariance matrix defined in terms of the same factor matrices $\Vmat$ and $\Phimat$ as the Krylov prior.

\begin{theorem}
  \label{T:KrylovPrior}
  The iterates resulting from $1\leq m \leq \kry$ iterations of BayesCG under the Krylov prior $\eta_0 = \N(\xvec_0,\Gammat_0)$ are  $\eta_i = \mathcal{N}(\xvec_i,\Gammat_i)$, $1\leq i \leq m$. The mean vectors $\xvec_i$, $1\leq i \leq m$, are equal to the CG iterates starting from the initial guess $\xvec_0$ and the covariance matrices are 
  \begin{align}
\label{Eq:GammaN}
\Gammat_{i} = \sum_{j = i+1}^\kry \phi_j \tilde{\vvec}_j\tilde{\vvec}_j^T = \Vmat_{i+1:\kry}\Phimat_{i+1:\kry}\left(\Vmat_{i+1:\kry}\right)^T, \qquad 1\leq i \leq m
\end{align}
where
\begin{align*}
  \Vmat_{i+1:\kry} = \begin{pmatrix} \tilde{\vvec}_{i+1}& \tilde{\vvec}_{i+2} & \cdots & \tilde{\vvec}_{\kry}\end{pmatrix}\quad \text{and} \quad  \Phimat_{i+1:\kry} = \mathrm{diag}\left(\phi_{i+1},\phi_{i+2},\ldots,\phi_\kry\right).
\end{align*}
\end{theorem}

\tref{T:KrylovPrior} holds for any $\Phimat$ with $\phi_i > 0$, $1\leq i \leq \kry$. The specific value of $\Phimat$ chosen in \dref{D:KrylovPrior} relates the posterior covariance $\Gammat_m$ to the error $\|\xvec_*-\xvec_m\|_\Amat^2$ \cite[Theorem 4.3]{RICO20}. The square $\Amat$-norm error $\|\xvec_*-\xvec_m\|_\Amat^2$ in CG, and also BayesCG under the Krylov prior, is equal to the sum of all remaining squared step lengths \cite[Theorem 6:1]{Hestenes} \cite[Section 5.6.1]{Liesen}. In terms of $\Phimat$ and the values in \aref{A:CG} this is
\begin{equation}
  \label{Eq:PhiTrace}
  \|\xvec_*-\xvec_m\|_\Amat^2 = \sum_{i=m+1}^\kry\gamma_i^2\|\rvec_i\|^2_2 = \sum_{i=m+1}^\kry\phi_i = \trace(\Phi_{m+1:\kry}), \qquad 1\leq m \leq \kry.
\end{equation}
This equation does not hold in finite precision arithmetic because it relies on the termination of CG in $\kry$ iterations. However, in \sref{S:KrylovApprox} we discuss an error estimate related to \eref{Eq:PhiTrace} that was shown to hold in finite precision arithmetic in \cite{StrakosTichy}.

Computing the Krylov prior is computationally expensive. Computing the $\kry$ vectors in the factor matrix $\Vmat$ requires as much computational effort as fully solving the the linear system. However, an approximation of the Krylov posterior can be efficiently computed. In the following section, we restate the definition of the approximate Krylov posterior from \cite[Section 3.2]{RICO20} and compute its approximation error in term of the Wasserstein distance.

\section{Krylov posterior properties}

\subsection{Approximation error}

A low rank approximation of the Krylov posterior can be computed a cost equal to a few additional iterations of CG, and in \cite[\textcolor{red}{SECTION}]{RIC020} it is shows that samples from the approximate Krylov posterior can produce a reliable error estimate. The downside of the approximate Krylov posterior is that $\xvec_*$ is not its support, the subset of $\Rn$ where the probability density function is not zero.

\textcolor{red}{I think I can remove the first paragraph}



\section{Assessing the Krylov Posterior}
\label{S:KrylovZS}

In this section, we discuss the performance of the Krylov posterior with the $Z$-statistic (\sref{S:KrylovZ}) and the $S$-statistic (\sref{S:KrylovS}). We show that both test statistics suggest the full-rank Krylov posterior is close to well calibrated and that the approximate Krylov posterior is optimistic.

\subsection{Z Statistic}
\label{S:KrylovZ}

In this section we assess the Krylov posterior with the $Z$-statistic. We compute the Moore-Penrose inverse of the Krylov posterior covariance (\lref{L:KrylovInv}), relate the error $\xvec_*-\xvec_m$ to the factor matrices of the Krylov posterior (\lref{L:KrylovErr}), then compute the $Z$-statistic for the Krylov posterior (\tref{T:KrylovZ}).

After stating a property of the Moore-Penrose inverse, we show the Moore-Penrose inverse of the Krylov posterior is computed with $\Amat$ and the Krylov posterior factor matrices $\Vmat$ and $\Phimat$.








We combine Lemmas \ref{L:KrylovInv}, \ref{L:KrylovErr}, and \ref{L:Phi} in the following theorem to compute the $Z$-statistic for BayesCG under the Krylov prior.


\subsection{Defintion of Z statistic}

The calibratedness of the BayesCG \cite{Cockayne:BCG} and BayesGMRES \cite{Bartels} posterior distributions was assessed with a test statistic called the $Z$-statistic. The $Z$-statistic, originally presented in \cite[Section 6.1]{Cockayne:BCG}, is derived by applying the the square Euclidean norm to the first expression in \eref{Eq:StrongCalibration}, and it relates a distribution of errors to a chi-square distribution. We restate the definition of the chi-square distribution (\dref{D:Chi2}) and $Z$-statistic (\tref{T:ZStat}) then discuss how it is used to assess a probabilistic linear solver (\aref{A:ZStat}).

\section{BayesCG Extras}

\begin{definition}[{\cite[Definition 6.2.4]{CM09}}]\label{d_1}
A (1,2) inverse of a matrix $\Emat\in\mathbb{R}^{k\times \ell}$ is a 
matrix $\Xmat\in\mathbb{R}^{\ell\times k}$ that satisfies the two conditions
\begin{equation*}
\Emat\Xmat\Emat=\Emat \qquad \text{and}\qquad \Xmat\Emat\Xmat=\Xmat.
\end{equation*}
We denote this (1,2) inverse by $\Emat^+=\Xmat$.
\end{definition}

Below is the explicit expression for the (1,2) inverse of an approximate 
Krylov posterior.

\begin{lemma}
  \label{L:KrylovInv12}
  Let $1\leq d\leq \kry-m$.
  The rank-$d$ approximate Krylov posterior covariance 
  $\widehat{\Gammat}_m = \Vmat_{m+1:m+d} \Phimat_{m+1:m+d} \,\Vmat_{m+1:m+d}^T$ in Definition~\ref{D:KrylovApprox} has a (1,2) inverse of the form
  \begin{equation*}
    \widehat{\Gammat}_m^{+} \equiv \Amat\Vmat_{m+1:m+d}\Phimat_{m+1:m+d}^{-1}\Vmat_{m+1:m+d}^T\Amat.
  \end{equation*}
\end{lemma}

\begin{proof}
Write the approximate posterior as a congruence
  \begin{equation}
   \label{Eq:L:KrylovInv}
\widehat{\Gammat}_m = \Amat^{-1/2}
    \underbrace{\Amat^{1/2}\Vmat_{m+1:m+d}\Phimat_{m+1:m+d}\Vmat_{m+1:m+d}^T\Amat^{1/2}}_{\Jmat}\Amat^{-1/2}.
  \end{equation}
 Here 
 \begin{align}
    \label{Eq:JSVD}
    \Jmat &\equiv \Amat^{1/2}\Vmat_{m+1:m+d}\Phimat_{m+1:m+d}\,
    \Vmat_{m+1:m+d}^T\,\Amat^{1/2}\notag\\
   & =\Zmat \,\Phimat_{m+1:m+d}\,\Zmat^T
      \end{align}
where $\Zmat\equiv \Amat^{1/2}\Vmat_{m+1:m+d}$
has orthonormal columns.
Since $\Phimat_{m+1:m+d}$ is non-negative diagonal, $\Jmat$
is symmetric positive semi-definite with eigenvalue decomposition 
and singular value decomposition (\ref{Eq:JSVD}), and Moore-Penrose inverse 
\begin{comment}
We express $\widehat{\Gammat}_m$ as a singular value decomposition multiplied by non-singular matrices. Define
   The columns of $\Amat^{1/2}\Vmat_{m+1:m+d}$ are orthonormal because the columns of $\Vmat$ are $\Amat$-orthonormal. As a consequence, \eref{Eq:JSVD} is a thin singular value decomposition\footnote{$\Jmat$ in \eref{Eq:JSVD} is equal to $\Jmat$ in the proof of \tref{T:Wasserstein}. $\Jmat$ is a symmetric positive semi-definite matrix because $\Phimat_{m+1:m+d}$ is a diagonal matrix with non-negative entries. The singular value decomposition of a symmetric positive semi-definite matrix is the same as its eigenvalue decomposition.} of $\Jmat$.
\end{comment}
  \begin{equation*}
    \Jmat^\dagger =\Zmat \, \Phimat_{m+1:m+d}^{-1}\, \Zmat^T=
  \Amat^{1/2}\Vmat_{m+1:m+d}\,\Phimat_{m+1:m+d}^{-1}\,\Vmat_{m+1:m+d}^T\,\Amat^{1/2}.
  \end{equation*}
The matrix
  \begin{align*}
    \widehat{\Gammat}_m^{+} = \Amat^{1/2}\Jmat^\dagger\Amat^{1/2} = \Amat\Vmat_{m+1:m+d}\,\Phimat_{m+1:m+d}^{-1}\,\Vmat_{m+1:m+d}^T\,\Amat
  \end{align*}
satisfies the properties in Definition~\ref{d_1}, with 
$\widehat{\Gammat}_m\widehat{\Gammat}_m^{+}
\widehat{\Gammat}_m=\widehat{\Gammat}_m$ and 
$\widehat{\Gammat}_m^{+}\widehat{\Gammat}_m\widehat{\Gammat}_m^{+}=\widehat{\Gammat}_m^{+}$, hence is 
a (1,2) inverse of $\widehat{\Gammat}_m$.
\qed \end{proof}

\begin{theorem}
%\label{T:CalibratedTrace}
  Let $\Amat\Xrv_* = \Brv$ be a random system of linear equations where $\Amat\in\R^{n\times n}$ is symmetric positive definite and $\Xrv_*\sim\mu_0 \equiv\N(\xvec_0,\Sigmat_0)$. Let $\mu_m \equiv \N(\xvec_m,\Sigmat_m)$, $1\leq m \leq \rank(\Sigmat_0)$ be the posterior distributions computed by the calibrated version of BayesCG. Then
  \begin{equation*}
    \Exp[\|\Xrv_* - \xvec_m\|_{\Sigmat_0^\dagger}^2] = \trace(\Sigmat_0^\dagger\Sigmat_m).
  \end{equation*}
  If additionally $\Sigmat_0 = \Amat^{-1}$, then
  \begin{equation*}
    \Exp[\|\Xrv_*-\xvec_m\|_\Amat^2] = \trace(\Amat\Sigmat_m).
  \end{equation*}
\end{theorem}

\begin{proof}
  This proof has multiple steps, and supplemental results are in the appendix.
  
  First, we show that $\|\Xrv_* - \xvec_m\|_{\Sigmat_0^\dagger}$ is distributed according to a chi-square distribution with $p = \rank(\Sigmat_0) - m$ degrees of freedom. Then, we show that $\trace(\Sigmat_0^\dagger\Sigmat_m) = p$. This completes the proof because the expected value of a chi-square distribution is equal to its degrees of freedom.

  \paragraph{Distribution of error.} To show that the error is distributed according to a chi-square distribution, we will show that the covariance of $(\Sigmat_0^\dagger)^{1/2}(\Xrv_* - \xvec_m)$ is an orthogonal projector and then invoke \lref{L:ChiProjector} from \appref{S:Aux}.

  This version of BayesCG is calibrated, therefore \lref{L:CalibrationAlt} implies
  \begin{equation*}
    (\Xrv_* - \xvec_m) \sim \N(\zerovec, \Sigmat_m).
  \end{equation*}
   Multiplying this equation on the left by $(\Sigmat_0^\dagger)^{1/2}\Sigmat_m^{1/2}\Umat^T$ results in
  \begin{equation}
    \label{Eq:HalfError}
    (\Sigmat_0^\dagger)^{1/2}(\Xrv_* - \xvec_m)\sim \N(\zerovec,\Pmat), \qquad \Pmat = (\Sigmat_0^\dagger)^{1/2}\Sigmat_m(\Sigmat_0^\dagger)^{1/2} 
  \end{equation}
  Denote by $\Tmat_m\in\R^{n\times m}$ the matrix whose columns are linearly independent search directions that do not depend on $\xvec_*$. Substituting \eref{Eq:SigmTheory} and $\Gmat = \Sigmat_0^{1/2}\Amat\Tmat_m$ into the formula for $\Pmat$ shows that
  \begin{align*}
    \Pmat &= (\Sigmat_0^\dagger)^{1/2}(\Sigmat_0 - \Sigmat_0 \Amat\Tmat_m(\Tmat_m^T\Amat\Sigmat_0\Amat\Tmat_m)^{-1}\Tmat_m^T\Amat\Sigmat_0)(\Sigmat_0^\dagger)^{1/2} \\
          &= \Imat - \Sigmat_0^{1/2}\Amat\Tmat_m(\Tmat_m^T\Amat\Sigmat_0\Amat\Tmat_m)^{-1}\Tmat_m^T\Amat\Sigmat_0^{1/2} \\
    &= \Imat - \Gmat(\Gmat^T\Gmat)^{-1}\Gmat,
  \end{align*}
  which is an orthogonal projector.

  Since the covariance matrix of \eref{Eq:HalfError} is an orthogonal projector, we apply \lref{L:ChiProjector} to get
  \begin{equation*}
    (\Xrv_*-\xvec_m)^T\Sigmat_0^\dagger(\Xrv_*-\xvec_m) = \|\Xrv_* - \xvec_m\|_{\Sigmat_0^\dagger}^2 \sim \chi_p^2.
  \end{equation*}

  \paragraph{Trace of the covariance.} We generalize \cite[Proposition 2]{Cockayne:BCG} to singular prior covariances to compute $\trace(\Sigmat_0^\dagger\Sigmat_m)$.

  From the cyclic commutativity of the trace, the linearity of the trace, and~\eref{Eq:SigmTheory} follows
  \begin{align}
    \trace(\Sigmat_0^\dagger\Sigmat_m) &= \trace(\Sigmat_0^\dagger(\Sigmat_0 - \Sigmat_m\Amat\Tmat_m(\Tmat_m^T\Amat\Sigmat_0\Amat\Tmat_m)^{-1}\Tmat_m^T\Amat\Sigmat_0)) \notag\\
                                       &= \trace(\Sigmat_0^\dagger\Sigmat_0) - \trace((\Tmat_m^T\Amat\Sigmat_0\Sigmat_0^\dagger\Sigmat_0\Amat\Tmat_m)(\Tmat_m^T\Amat\Sigmat_0\Amat\Tmat_m)^{-1}) \notag\\
    &= \rank(\Sigmat_0) - m. \label{Eq:TraceRank}
  \end{align}

  \paragraph{Expected value of the error.} The expected value of a chi-square distribution is equal to its degrees of freedom. Therefore, 
  \begin{equation*}
    \Exp[\|\Xrv_*-\xvec_m\|_{\Sigmat_0^\dagger}^2] = \rank(\Sigmat_0) - m.
  \end{equation*}
  \qed
\end{proof}

\subsubsection{Numerical rank}

In $Z$-statistic experiments, we use the median numerical rank of the posterior covariance for the chi-square distribution's degrees of freedom. This is because the numerical rank of $\Sigmat_m$ can differ from
\begin{equation*}
  \rank(\Sigmat_m) = \rank(\Sigmat_0) - m.
\end{equation*}
Additionally, the value of $\kry$ in finite precision depends on the termination criterion chosen in BayesCG under the Krylov prior.

The numerical rank of $\Sigmat_m$ is
\begin{equation*}
  \rank(\Sigmat_m) = \mathrm{cardinality} \{\sigma_i \ | \ \sigma_i > n\varepsilon \|\Sigmat_m\|_2\},
\end{equation*}
where $\varepsilon$ is machine epsilon and $\sigma_i$, $1\leq i \leq n$ are the singular values of $\Sigmat_m$ \cite[Section 5.4.1]{GoVa13}\footnote{This rank formula is used in the Matlab function \texttt{rank} and the NumPy function \texttt{numpy.linalg.rank}.}.


==> UQZSStats.tex <==
\section{Assessing the Posterior Distribution with the $Z$-statistic}
\label{S:UQZ}

In this section we discuss the $Z$-statistic, an existing method of assessing whether $\mu_m$ is well calibrated.  We restate in \sref{S:ZDef} the definition of the $Z$-statistic and discuss how it is used, and we summarize in \sref{S:ZBayesCG} the $Z$-statistic experiments from \cite{Cockayne:BCG} assessing the BayesCG posterior.

\subsection{Definition and Use of the $Z$-statistic}
\label{S:ZDef}

The calibratedness of the BayesCG \cite{Cockayne:BCG} and BayesGMRES \cite{Bartels} posterior distributions was assessed with a test statistic called the $Z$-statistic. The $Z$-statistic, originally presented in \cite[Section 6.1]{Cockayne:BCG}, is derived by applying the the square Euclidean norm to the first expression in \eref{Eq:StrongCalibration}, and it relates a distribution of errors to a chi-square distribution. We restate the definition of the chi-square distribution (\dref{D:Chi2}) and $Z$-statistic (\tref{T:ZStat}) then discuss how it is used to assess a probabilistic linear solver (\aref{A:ZStat}).

\begin{definition}{{\cite[Definition 2.2]{Ross07}}}
  \label{D:Chi2}
  The chi-square distribution with $p$ degrees of freedom is the distribution of
  \begin{equation*}
    \Xrv^T\Xrv\sim\chi_p^2,
  \end{equation*}
  where $\Xrv\sim\N(\zerovec,\Imat_p)$.
\end{definition}

\begin{theorem}[{\cite[Section 6.1]{Cockayne:BCG}, \cite[Proposition 1]{BCG:Supp}}]
    \label{T:ZStat}
  The $Z$-statistic for the solution $\xvec_*$ of \eref{Eq:Axb} is 
  \begin{equation*}
    \Zstat(\xvec_*) = (\xvec_*-\xvec_m)^T\Sigmat_m^\dagger(\xvec_*-\xvec_m).
  \end{equation*}
  If $\mu_m$ is calibrated in the sense of \dref{D:StrongCalibration} then the $Z$-statistic is distributed according to the chi-square distribution with $\rank(\Sigmat_m) = \rank(\Sigmat_0) - m$ degrees of freedom.
\end{theorem}

The process of computing $Z$-statistic samples is presented in \aref{A:ZStat}. The inputs of \aref{A:ZStat} are a matrix $\Amat$, an input distribution $\mu_0 = \N(\xvec_0,\Sigmat_0)$, a probabilistic linear solver that produces Gaussian posteriors \texttt{solver}, a reference distribution $\mu_{\text{ref}}$, the number of iterations to run the solver $m$, and the number of test problems $N_{\text{test}}$.

\begin{algorithm}
\caption{Sampling the $Z$-statistic}
\label{A:ZStat}
\begin{algorithmic}[1]
  \State \textbf{Input:} $\Amat\in\Rnn$, $\mu_0 = \N(\xvec_0,\Sigmat_0)$, \texttt{solver}, $\mu_{\text{ref}}$, $m$, $N_{\text{test}}$
  \For{$i = 1:N_{\text{test}}$}
  \State{Draw $\xvec_*$ from reference distribution $\mu_{\text{ref}}$} 
  \State{$\bvec = \Amat\xvec_*$} \Comment{Define test problem}
  \State{$\mu_m = \texttt{solver}(\Amat,\bvec,\mu_0,m)$} \Comment{Compute posterior $\mu_m = \N(\xvec_m,\Sigmat_m)$}
  \State{Compute $\Sigmat_m^\dagger$, the Moore-Penrose inverse of $\Sigmat_m$}
  \State{$ z_i = (\xvec_*-\xvec_m)^T\Sigmat_m^\dagger(\xvec_*-\xvec_m)$} \Comment{Compute $Z$-statistic sample}
  \EndFor
  \State{\textbf{Output:} Return $Z$-statistic samples $z_i$, $1\leq i \leq N_{test}$.}
\end{algorithmic}
\end{algorithm}

The test problems are generated by drawing a solution $\xvec_*$ from the reference distribution $\mu_{\text{ref}}$ with the right hand side vector computed as $\bvec = \Amat\xvec_*$. The reference distribution is usually equal to the prior distribution to satisfy the assumption that the prior distribution models the solution \cite[Section 6.4]{Bartels}. However, it is not always possible to use the prior distribution as the reference distribution, and in these cases some other reference distribution is chosen.

The calibratedness of a probabilistic linear solver is assessed with the $Z$-statistic by comparing $Z$-statistic samples generated by \aref{A:ZStat} to the chi-square distribution with $\rank(\Sigmat_0)-m$ degrees of freedom. As in \cite{Cockayne:BCG} and \cite{Bartels}, we primarily compare the $Z$-statistic and chi-square distributions visually. A visual comparison is sufficient because the non-equality of distributions is usually obvious, as can be seen in \cite[Figures 3 and 4]{Cockayne:BCG}, \cite[Figure 2]{Bartels}, and \sref{S:Experiments} of this paper. In \sref{S:Experiments}, we also compare the means of the $Z$-statistic chi-square distributions; however, we also note that comparing means is not sufficient to prove to distributions are equal. There are more rigorous methods of comparing the distributions, such as a Kolmogorov–Smirnov test, but we leave these methods for future work.

Comparing the of $Z$-statistic samples to the chi-square distribution tells us whether the posterior distribution $\mu_m$ is well calibrated, is pessimistic, or is optimistic.
\begin{description}
\item[\bf Well Calibrated] If $\mu_m$ is well calibrated, then the $Z$-statistic samples are distributed according to the chi-square distribution.
\item[\bf Pessimistic] If the $Z$-statistic samples are concentrated around smaller values than the chi-square distribution, then $\mu_m$ is \emph{pessimistic} \cite[Section 6.1]{Cockayne:BCG}, which means it is predicts $\xvec_*$ is in a larger area of $\Rn$ than it should. 
\item[\bf Optimistic] If the $Z$-statistic samples are concentrated around larger values than the chi-square distribution, then $\mu_m$ is \emph{optimistic} \cite[Section 6.1]{Cockayne:BCG}, which means it is predicts $\xvec_*$ is in a smaller area of $\Rn$ than it should. 
\end{description}


\subsection{$Z$-statistic experiments in existing work}
\label{S:ZBayesCG}

We summarize the results of the BayesCG $Z$-statistic experiments in \cite{Cockayne:BCG} and discuss factors that affect the quality the BayesCG posterior distribution. 

\paragraph{$Z$-statistic and the BayesCG posterior} Numerical experiments to determine if the BayesCG posterior is well calibrated were performed in \cite[Section 6.1]{Cockayne:BCG}. These experiments show that the BayesCG posterior distribution is \emph{conservative}, it models $\xvec_*$ as being in a larger subset of $\R^\dm$ than what the error indicates is reasonable.

The BayesCG posterior distribution is conservative because \tref{T:XmSigmTheory} assumes $\Yrv_m = \Smat_m^T\Amat\xvec_*$ depends linearly on $\xvec_*$, while in \aref{A:BayesCG} the initial search direction is the residual $\rvec_0 = \Amat(\xvec_*-\xvec_0)$, causing $\Yrv_m$ to be non-linearly dependent on $\xvec_*$. As a consequence, the posterior mean and covariance formulas in \tref{T:XmSigmTheory} rely on a linear approximation of $\Yrv_m$. The effect the linear approximation has on the posterior is that $\Sigmat_m$ converges to $\zerovec$ more slowly than $\xvec_m$ converges to $\xvec_*$.

\paragraph{Prior Choice and quality of BayesCG posterior} The quality of the BayesCG posterior is affected by the choice of prior covariance. The choices of prior covariance examined in \cite[Sections 4.1 and 6.1]{Cockayne:BCG} are:
\begin{itemize}
\item $\Sigmat_0 = \Imat$, which is easy to compute
\item $\Sigmat_0 = \Amat^{-1}$, which causes the BayesCG mean vector iterates to be equal to the CG iterates
\item $\Sigmat_0 = \left(\Pmat^T\Pmat\right)^{-1}$ where $\Pmat \approx \Amat$ is a preconditioner for \eref{Eq:Axb}
\item ``Krylov Subspace Prior'' where $\Sigmat_0$ depends on the Krylov subspace used in BayesCG
\end{itemize}
In the experiments in \cite[Section 6.1]{Cockayne:BCG}, the prior covariance that caused the distribution of $Z$-statistic samples to be closest to the chi-squared distribution was the Krylov subspace prior, followed by the identity, inverse, and preconditioner priors.

\paragraph{Scale of BayesCG posterior} The scale of the posterior covariance affects calibratedness of the posterior distribution. Scaling the posterior covariance is proposed in \cite[Section 4.2]{Cockayne:BCG} to improve the calibratedness of the BayesCG posterior distribution. Scaling the posterior has also been proposed to improve the calibratedness of matrix based inference methods \cite[Section 3]{WH20}. The scale can be determined in a hierarchical Bayesian procedure \cite[Proposition 11]{Cockayne:BCG} or through a heuristic procedure \cite[Section S4.3]{BCG:Supp} \cite[Section 3]{WH20}. 

The heuristic scale examined in \cite[Section S4.3]{BCG:Supp} is an estimate of the error $\|\xvec_*-\xvec_m\|_2^2$. Scaling the posterior with the error estimate made the size of the area the posterior is concentrated proportional to the error, and this improved the calibratedness of the posterior.

In \sref{S:Krylov} we construct a modification of the Krylov subspace prior that causes BayesCG to produce a well calibrated posterior. Our version of the Krylov prior also causes the posterior to have a scale related to the $\Amat$-norm error $\|\xvec_*-\xvec_m\|_\Amat^2$. However, we introduce a new test statistic related to the $\Amat$-norm error before constructing our version of the Krylov prior.

\section{Assessing the Posterior Distribution with the $S$-statistic}
\label{S:UQS}

We introduce the $S$-statistic as an alternative test statistic to the $Z$-statistic. The $S$-statistic is used to assess whether the posterior distribution of a probabilistic linear solver accurately models the solution. We construct the $S$-statistic in \sref{S:SStat} as an estimator of the Wasserstein distance between the posterior distribution and the solution, which we compute in \sref{S:Wasserstein}. 

The the $S$-statistic presented here is related to the CG error estimating $S$-statistic in \cite[Section 4.2]{RICO20}.  We chose to estimate the Wasserstein metric with this version of the $S$-statistic to allow us to quantify the relationship between the posterior and the solution.

Our motivation for creating the $S$-statistic was to assist in creating a prior that causes BayesCG to compute a well calibrated posterior. Additionally, the $S$-statistic has two advantages over the $Z$-statistic:
\begin{enumerate}
\item The $S$-statistic can be tested with 1 solution $\xvec_*$ instead of requiring a set of test problems and
\item If the posterior is calibrated, the $S$-statistic provides a computable estimate of the Wasserstein distance between the posterior and solution, which is more informative than the $\Sigmat^\dagger_m$-norm error estimated by the $Z$-statistic.
\end{enumerate}

\begin{comment}
\subsection{Wasserstein Distance}
\label{S:Wasserstein}

The Wasserstein distance is a metric on the set of probability distributions \cite[Chapter 6]{Villani09}. We compute a weighted Wasserstein distance between the solution $\xvec_*$ and the posterior distribution of a probabilistic linear solver in \eref{Eq:WassersteinAError}. In order to compute \eref{Eq:WassersteinAError}, we first state the definition of the Wasserstein metric (\dref{D:Wasserstein}) and derive a formula for a weighted Wasserstein metric between two Gaussian distributions (\lref{L:WassersteinNorm}).

\begin{definition}[{$p$-Wasserstein Distance \cite[Definition 2.1]{KLMU20}\cite[Definition 6.1]{Villani09}}]
  \label{D:Wasserstein}
  Let $\mu$ and $\nu$ be two probability distributions on $\Rn$. The $p$-Wasserstein distance between $\mu$ and $\nu$ is
\begin{equation}
  \label{Eq:WassersteinInt}
  W_p(\mu,\nu) =  \left(\inf_{\pi\in\Pi(\mu,\nu)}\int_{\Rn\times\Rn}\|\Mrv-\Nrv\|_2^p \ d\pi(\Mrv,\Nrv)\right)^{1/p} , \quad p\geq 1,
\end{equation}
where $\Pi(\mu,\nu)$ is the set of couplings of $\mu$ and $\nu$, the set of probability distributions on $\Rn\times\Rn$ that have $\mu$ and $\nu$ as marginal distributions.
\end{definition}

The $2$-Wasserstein distance, also known as the Frech\'{e}t distance, between two Gaussian distributions can be computed with the formula dependent on the means and covariances of the two distributions \cite{Gelbrich90}.

\begin{lemma}[{\cite[Theorem 2.1]{Gelbrich90}}]
  \label{L:2Wasserstein}
  Let $\mu = \N(\xvec_\mu,\Sigmat_\mu)$ and $\nu = \N(\xvec_\nu,\Sigmat_\nu)$ be two Gaussian distributions on $\Rn$. The 2-Wasserstein distance between $\mu$ and $\nu$ is
  \begin{equation*}
    W_2(\mu,\nu) = \left(\|\xvec_\mu-\xvec_\nu\|_2^2 + \trace\left[\Sigmat_\mu+\Sigmat_\nu - 2\left(\Sigmat_\mu^{1/2}\Sigmat_\nu\Sigmat_\mu^{1/2}\right)^{1/2}\right]\right)^{1/2}.
  \end{equation*}
\end{lemma}

In the following theorem we define the $\Bmat$-Wasserstein distance and adapt the formula in \lref{L:2Wasserstein} to show it can be computed easily when comparing Gaussian distributions. The main idea of the theorem is to apply the stability property of Gaussian distributions---linear transformations of Gaussian distributions are also Gaussian \cite[Section 1.2]{Muirhead}---to express the $\Bmat$-Wasserstein distance as a $2$-Wasserstein distance.

\begin{theorem}
  \label{L:WassersteinNorm}
  Let $\mu = \N(\xvec_\mu,\Sigmat_\mu)$ and $\nu = \N(\xvec_\nu,\Sigmat_\nu)$ be two Gaussian distributions on $\Rn$, and let $\Bmat\in\Rnn$ be a symmetric positive definite matrix. We define the $\Bmat$-Wasserstein distance as
  \begin{align}
    \label{Eq:L:WassersteinNorm:Exp}
    W_\Bmat (\mu,\nu) &= \left(\inf_{\pi\in\Pi(\mu,\nu)}\int_{\Rn\times\Rn}\|\Mrv-\Nrv\|_\Bmat^2 \ d\pi(\Mrv,\Nrv)\right)^{1/2},
  \end{align}
  where
  \begin{equation}
    \label{Eq:BNorm}
    \|\xvec\|_\Bmat = \|\Bmat^{1/2}\xvec\|_2, \quad \xvec\in\Rn,
  \end{equation}
  is the vector $\Bmat$-norm. Then,
  \begin{align}
    \label{Eq:WassersteinNormA}
    \left[W_\Bmat(\mu,\nu)\right]^2 &= \|\xvec_\mu-\xvec_\nu\|_\Bmat^2 + \trace[\Bmat\Sigmat_\mu]+\trace[\Bmat\Sigmat_\nu]  \\ 
    &-2\trace[((\textcolor{red}{\Bmat^{1/2}\Sigmat_\mu \Bmat^{1/2}})^{1/2}\textcolor{blue}{\Bmat^{1/2}\Sigmat_\nu \Bmat^{1/2}}(\textcolor{red}{\Bmat^{1/2}\Sigmat_\mu \Bmat^{1/2}})^{1/2})^{1/2}]. \notag
  \end{align}
\end{theorem}

\begin{proof}
  The main idea of this proof is to express \eref{Eq:L:WassersteinNorm:Exp} as a 2-Wasserstein distance and apply the 2-Wasserstein distance formula from \lref{L:2Wasserstein}.

  Substituting \eref{Eq:BNorm} into \eref{Eq:L:WassersteinNorm:Exp} gives
  \begin{equation}
    \label{Eq:BWassersteinExp}
    W_\Bmat(\mu,\nu) = \left(\inf_{\pi\in\Pi(\mu,\nu)}\int_{\Rn\times\Rn}\|\Bmat^{1/2}\Mrv - \Bmat^{1/2}\Nrv\|_2^2 \ d\pi(\Mrv,\Nrv)\right)^{1/2}.
  \end{equation}
  Because of the stability of Gaussian distributions \cite[Section 1.2]{Muirhead}, $\Bmat^{1/2}\Mrv$ and $\Bmat^{1/2}\Nrv$ are Gaussian random variables distributed according to
  \begin{equation*}
    \bar{\mu} = \mathcal{N}(\Bmat^{1/2}\xvec_\mu,\Bmat^{1/2}\Sigmat_\mu\Bmat^{1/2}) \quad \text{and} \quad  \bar{\nu} = \mathcal{N}(\Bmat^{1/2}\xvec_\nu,\Bmat^{1/2}\Sigmat_\nu\Bmat^{1/2})
  \end{equation*}
  respectively. As a consequence, \eref{Eq:BWassersteinExp} can be expressed as the 2-Wasserstein distance
  \begin{align*}
    W_\Bmat(\mu,\nu) &= \left(\inf_{\pi\in\Pi(\bar{\mu},\bar{\nu})}\int_{\Rn\times\Rn}\|\bar{\Mrv} - \bar{\Nrv}\|_2^2 \ d\pi(\bar{\Mrv},\bar{\Nrv})\right)^{1/2} \\
    &= W_2(\bar{\mu},\bar{\nu}).
  \end{align*}
  Applying \lref{L:2Wasserstein} to the previous equation and simplifying with the cyclic commutativity and linearity of the trace results in \eref{Eq:WassersteinNormA}.
  \qed \end{proof}

\end{comment}

With \lref{L:WassersteinNorm}, we compute the $\Bmat$-norm Wasserstein metric between the posterior distribution $\mu_m = \mathcal{N}(\xvec_m,\Sigmat_m)$ and a Dirac distribution at the solution $\xvec_*$ as
\begin{equation}
  \label{Eq:WassersteinAError}
  \left[W_\Bmat(\mu_m,\xvec_*)\right]^2 = \|\xvec_m-\xvec_*\|_\Bmat^2 + \trace(\Bmat\Sigmat_m).
\end{equation}
The Dirac distribution at $\xvec_*$ in \eref{Eq:WassersteinAError} is modeled as $\N(\xvec_*,\zerovec)$. For BayesCG we set the weight matrix in \eref{Eq:WassersteinAError} to be $\Bmat = \Amat$ to relate the BayesCG $\Amat$-Wasserstein error to the CG $\Amat$-norm error.

In the following section, we construct the $S$-statistic so that it estimates~\eref{Eq:WassersteinAError}.

\subsection{S Statistic}
\label{S:SStat}

We construct the $S$-statistic as a sampling method that estimates the $\Bmat$-Wasserstein distance between the posterior distribution $\mu_m$ and the  solution $\xvec_*$. To do this, we first define a general form of the $S$-statistic as the difference between two random vectors (\dref{D:SGen}) and compute its expected value (\lref{L:ExpS}). We then define the specific versions of the $S$-statistic for probabilistic linear solvers (\dref{D:SBayesCG}).

\begin{definition}[$S$-statistic]
  \label{D:SGen}
Let $\mu = \N(\xvec_\mu,\Sigmat_\mu)$ and $\nu = \N(\xvec_\nu,\Sigmat_\nu)$ be Gaussian distributions, and let $\Bmat$ be a symmetric positive definite matrix. The $S$ statistic is
\begin{equation*}
\Sstat_\Bmat (\mu,\nu) := \|\Mrv-\Nrv\|_\Bmat^2 = \left(\Mrv-\Nrv\right)^T\Bmat\left(\Mrv-\Nrv\right),
\end{equation*}
where $\Mrv\sim\mu$ and $\Nrv\sim\nu$ are independent random variables.
\end{definition}

The $S$-statistic is a quadratic form because it is the weighted inner product of a random variable with itself. The expected value of a quadratic form can be computed analytically, which we state in the following lemma.

\begin{lemma}[Sections 3.2b.1--3.2b.3 in \cite{Mathai}]
  \label{L:QuadExp}
  Let $\Zrv\sim\N(\xvec_z,\Sigmat_z)$ be a random variable, and let $\Bmat\in\Rnn$ be symmetric positive definite. 
  The mean  of $\Zrv^T\Bmat\Zrv$ is
  \begin{align*}
    \Exp[\Zrv^T\Bmat\Zrv] &= \trace(\Bmat\Sigmat_z) + \xvec_z^T\Bmat\xvec_z.
  \end{align*}
\end{lemma}

We now compute the expected value of the $S$-statistic by applying \lref{L:QuadExp}.

\begin{lemma}
\label{L:ExpS}
The expected value of the $S$-statistic from \dref{D:SGen} is 
\begin{equation}
\label{Eq:SMean}
\mathbb{E}\left[\Sstat_\Bmat (\mu,\nu)\right] = \trace(\Amat(\Sigmat_\mu+\Sigmat_\nu)) + \|\xvec_\mu-\xvec_\nu\|_\Amat^2.
\end{equation}
\end{lemma}

\begin{proof}
  In order to apply \lref{L:QuadExp}, we compute the mean and covariance of $\Mrv-\Nrv$ from \dref{D:SGen}. The mean of $\Mrv-\Nrv$ is
\begin{equation}
  \label{Eq:SMean}
\mathbb{E}(\Mrv-\Nrv) = \xvec_\mu-\xvec_\nu.
\end{equation}
The covariance of $\Mrv-\Nrv$ is
\begin{align}
  \Sigmat_{\Mrv-\Nrv}&:=\mathrm{Cov}(\Mrv-\Nrv,\Mrv-\Nrv) \\
                     &= \mathbb{E}\left[\left((\Mrv-\xvec_\mu)-(\Nrv-\xvec_\nu)\right)\left((\Mrv-\xvec_\mu)-(\Nrv-\xvec_\nu)\right)^T\right] \notag\\
&= \mathrm{Cov}(\Mrv,\Mrv) + \mathrm{Cov}(\Nrv,\Nrv) -\mathrm{Cov}(\Mrv,\Nrv) - \mathrm{Cov}(\Nrv,\Mrv). \label{Eq:SCov}
\end{align}
The last two covariance terms in \eref{Eq:SCov} are $\mathrm{Cov}(\Mrv,\Nrv) =\mathrm{Cov}(\Nrv,\Mrv) = 0$ because $\Mrv$ and $\Nrv$ are independent.

From \lref{L:QuadExp}, \eref{Eq:SMean}, and \eref{Eq:SCov} follows
\begin{align*}
\mathbb{E}\left[\Sstat_\Bmat (\mu,\nu)\right] = \trace(A(\Sigmat_z+\Sigmat_\nu)) + \|\xvec_\mu-\xvec_\nu\|_\Amat^2.
\end{align*}
\qed \end{proof}

We define two specific versions of the $S$-statistic for probabilistic linear solvers. These versions are to assess the quality of the posterior distribution and estimate the $\Bmat$-Wasserstein distance between the posterior distribution and the solution.

\begin{definition}[Solution and Computable $S$-statistics]
  \label{D:SBayesCG}
  Let $\mu_m$ be the posterior distribution of a probabilistic linear solver, and let $\Bmat$ be a symmetric positive definite matrix. We define the \emph{solution $S$-statistic} as
  \begin{equation*}
    \Sstat_\Bmat(\mu_m,\xvec_*) = \|\Xrv-\xvec_*\|_\Bmat^2,
  \end{equation*}
  and we define the \emph{computable $S$-statistic} as
  \begin{equation*}
    \Sstat_\Bmat(\mu_m,\mu_m) = \|\Xrv-\Xrv'\|_\Bmat^2,
  \end{equation*}
  where $\Xrv, \Xrv'\sim\mu_m$ are independent random variables distributed according to $\mu_m$.
\end{definition}

By \lref{L:ExpS}, the expected value of the solution $S$-statistic is
\begin{equation}
  \label{Eq:ExpS}
  \mathbb{E}\left[\Sstat_\Bmat (\mu_m,\xvec_*)\right] = \|\xvec_m-\xvec_*\|_\Bmat^2 + \trace(\Bmat\Sigmat_m)
\end{equation}
and the expected value of the computable $S$-statistic is
\begin{equation}
  \label{Eq:ExpAltS}
  \mathbb{E}\left[\Sstat_\Bmat (\mu_m,\mu_m)\right] = 2\trace(\Bmat\Sigmat_m).
\end{equation}
Equations \eref{Eq:ExpS} and \eref{Eq:WassersteinAError} show that the expected value of the solution $S$-statistic, $\Sstat(\mu_m,\xvec_*)$, is equal to the $\Bmat$-norm Wasserstein metric between the posterior distribution and true solution.

The computable $S$-statistic should have the same distribution as the $S$-statistic if the posterior distribution $\mu_m$ is calibrated in the sense of \dref{D:StrongCalibration}. If $\mu_m$ is well calibrated, then $\xvec_*\sim\mu_m$ and the $S$-statistic and the computable $S$-statistic are the same. Therefore, the calibratedness of $\mu_m$ can be assessed by comparing the distributions of the $S$-statistic and the Computable $S$-statistic.

The process of sampling the solution and computable $S$-statistics is outlined in \aref{A:SStat}. The inputs to \aref{A:SStat} are the solution $\xvec_*$, the symmetric positive definite matrix $\Bmat$, the posterior distribution $\mu_m$, and the number of samples $N_{sample}$. The main idea of \aref{A:SStat} is to compute the distributions of both versions of the Wasserstein $S$-statistic with sampling.

\begin{algorithm}
\caption{Sampling $S$-statistic}
\label{A:SStat}
\begin{algorithmic}[1]
  \State \textbf{Input:} $\xvec_*$, $\Bmat\in\Rnn$, $\mu_m = \N(\xvec_0,\Sigmat_0)$, $N_{\text{samples}}$
  \For{$i = 1:N_{\text{samples}}$}
  \State{Draw $\uvec$ and $\yvec$ from posterior distribution $\mu_{m}$} 
  \State{$ s_i = (\uvec-\xvec_*)^T\Bmat(\uvec-\xvec_*)$} \Comment{Sample Solution $S$-statistic}
  \State{$ c_i = (\uvec-\yvec)^T\Bmat(\uvec-\yvec)$} \Comment{Sample Computable $S$-statistic}
  \EndFor
  \State{\textbf{Output:} Samples of solution and computable $S$-statistics:  $s_i$ and $c_i$, $1\leq i \leq N_{\text{samples}}$}
\end{algorithmic}
\end{algorithm}

Similarly to the $Z$-statistic, the distributions of both versions of the $S$-statistic are compared visually and by comparing their means. The relation between both versions of the $S$-statistic tell us whether the posterior distribution $\mu_m$ well calibrated, pessimistic, or optimistic.
\begin{description}
\item[\bf Well Calibrated] If $\mu_m$ accurately models $\xvec_*$ then $\Xrv\sim\mu_m$ approximates $\xvec_*$, causing the solution $S$-statistic $\Sstat_\Bmat(\mu_m,\xvec_*)$ and computable $S$-statistic $\Sstat_\Bmat(\mu_m,\mu_m)$ to have the same distribution.
\item[\bf Pessimistic] If $\mu_m$ is pessimistic then it is concentrated in a larger area of $\Rn$ than it should be. This causes samples of $\Xrv\sim\mu$ and $\Xrv'\sim\mu$ to be further from each other than $\Xrv$ and $\xvec_*$, causing  $\Sstat_\Bmat(\mu_m,\xvec_*)$ to be concentrated around smaller values than $\Sstat_\Bmat(\mu_m,\mu_m)$.
\item[\bf Optimistic] If $\mu_m$ is optimistic then it is concentrated in a smaller area of $\Rn$ than it should be. This causes samples of $\Xrv\sim\mu$ and $\Xrv'\sim\mu$ to be closer to each other than $\Xrv$ and $\xvec_*$, causing $\Sstat_\Bmat(\mu_m,\xvec_*)$ to be concentrated around larger values than $\Sstat_\Bmat(\mu_m,\mu_m)$.
\end{description}

\subsection{Comparing the $S$-statistic to the $Z$-statistic}

We now briefly compare the $Z$-statistic and the $S$-statistic. Both test statistics can assess whether a posterior distribution is well calibrated, pessimistic, or optimistic. 

\begin{figure}
  \centering
  \includegraphics[scale = .35]{Images/NotCalibrated}
  \includegraphics[scale = .35]{Images/CalibratedS} \\
  \includegraphics[scale = .35]{Images/CalibratedZS}
  \caption{Comparison of how $Z$-statistic and $S$-statistic would assess how well each distribution models solution ``X''. Both test statistics would indicate the top left distribution is not well calibrated. The $S$-statistic would indicate the top right distribution is well calibrated but the $Z$-statistic would not. Both test statistics would indicate the bottom distribution is well calibrated.}
  \label{F:ZSComparison}
\end{figure}

The $S$-statistic focuses primarily on the size of the area the posterior is concentrated in. As a consequence, the $S$-statistic can indicate distributions are calibrated when they are not. The $Z$-statistic is less likely to encounter this problem. An example of this situation is shown in \figref{F:ZSComparison}.

While the $Z$-statistic is better at assessing calibration, the $S$-statistic has some computational advantages over the $Z$-statistic. The $S$-statistic requires only one test problem while the $Z$-statistic requires a reference distribution to create a set of many test problems. The $S$-statistic is computationally faster because it does not compute a Moore-Penrose inverse for every test problem while the $Z$-statistic does. Finally, if the posterior is calibrated, the $S$-statistic produces a computable estimate of the Wasserstein distance between the posterior and the solution.


\section{Extras}

\section*{\textcolor{red}{Weak Calibration Notes}}

\textcolor{red}{BEGIN COMMENT}

I believe I have a proof that BayesCG under the Krylov prior is weakly calibrated. In this section I will define weak calibration (this definition will be from the pushforward paper), I will define the Weak Z statistic, and then I will show the BayesCG under the Krylov prior is weakly calibrated with the Weak Z statistic.

If this works, I intend this text to be put in the earlier sections
\begin{itemize}
\item The definition of weak calibration will go after the definition of strong calibration
\item The weak Z statistic will be in its own section after the Z statistic section. I intend this section to be similar to the existing Z statistic section
\item The weak calibration argument requires a new interpretation of BayesCG under the Krylov prior. This interpretation is that BayesCG under the Krylov prior is a version of BayesCG under the inverse prior that produces a scaled posterior distribution.
\end{itemize}

Since I intend this text to go into earlier sections, I will write it like it is in earlier sections

\textcolor{red}{END COMMENT}

\subsection*{Calibration}

\textcolor{DarkGreen}{\dref{D:StrongCalibration} requires the covariance matrix $\Sigmat_m$ be independent of $\Brv$, 
which means it is the same for every right hand side. This is a realistic constraint for stationary iterative methods. However, 
in BayesCG the covariance matrices $\Sigmat_m$ depend on 
the right-hand side through the search directions $\Smat_m$ and conditioning on $\Smat_m^T\Amat\Xrv = \Smat_m^T\Brv$. Therefore we
cannot apply \dref{D:StrongCalibration} directly to BayesCG.
However in \sref{S:UQZ}, we assess the calibration of BayesCG under the Krylov prior with the $Z$-statistic, a test statistic which can be derived from \dref{D:StrongCalibration} and has been used to assess the calibration
the calibration of Bayesian probabilistic linear solvers 
\cite[Section 6.1]{Cockayne:BCG}, \cite[Section 6.4]{Bartels}.} Additionally, we present a weaker form of calibration that does not require $\Sigmat_m$ be independent of $\Brv$.

\begin{definition}{{\cite[Definition 12]{CIOR20}}}
  \label{D:WeakCalibration}
  Given an symmetric positive definite matrix $\Amat\in\R^{n\times n}$,
  consider the class of linear systems $\Amat\Xrv = \Brv$ with random right hand side $\Brv\in\R^n$ defined by a random solution 
  $\Xrv\sim \mu_0$.
  
 A probabilistic linear solver for $\Amat\Xrv=\Brv$ that computes the posterior $\mu_m$ in $m \leq n$ iterations 
 is \textit{weakly calibrated} if the random variable $\Mrv \ | \Xrv \sim \mu_m$ has the marginal distribution $\Mrv \sim \mu_0$.
\end{definition}

\dref{D:WeakCalibration} means that a probabilistic linear solver is weakly calibrated if the average of the posterior distributions it computes in $m\leq n$ iterations for many randomly generated problems is equal to the prior distribution \cite[Section 1.1]{CIOR20}.

\begin{remark}
  \label{R:WeakCalibration}
  We test whether a linear solver is weakly calibrated with the following process \cite[Remark 13]{CIOR20}:
\begin{enumerate}
\item Generate a random linear system by sampling a solution from the prior $\mu_0$.
\item Run the solver for $m\leq n$ iterations to compute the posterior distribution $\mu_m$.
\item Sample a value from the posterior distribution
\item Repeat the above three steps several times. If the samples from the posterior distributions are distributed according to the prior, then the method is weakly calibrated.
\end{enumerate}
\end{remark}
In \textcolor{red}{section}, we adapt this process to develop a test statistic to assess whether a solver is weakly calibrated.

\paragraph{Relationship between strong and weak calibration} Strong calibration is stronger than weak calibration. All strongly calibrated probabilistic numerical methods are also weakly calibrated, but not all weakly calibrated methods are strongly calibrated \cite[Section 2.4.1]{CGOS21}. \textcolor{red}{ideas for additional comment: Strong calibration means that, on average, the solution we attempt to model with the posterior distribution is distributed according to the posterior distribution. Weak calibration means that, on average, samples from the posterior distribution are distributed according to the prior distribution.} 

\paragraph{Examples of calibration}

\textcolor{DarkGreen}{Adapt the examples to differentiate strong and weak calibration}

\subsection*{Assessing whether BayesCG  is weakly calibrated}

In this section, we assess whether BayesCG under the Krylov prior is weakly calibrated. First, we introduce the Weak $Z$-statistic, a test statistic to determine whether probabilistic linear solvers are weakly calibrated (\textcolor{red}{theorem}). Then we apply the Weak $Z$-statistic to BayesCG under the Krylov prior (\textcolor{red}{theorem}).

In the following theorem, we adapt the $Z$-statistic and \rref{R:WeakCalibration} into the Weak $Z$-statistic.

\begin{theorem}
  \label{T:WeakZ}
  Let $\mu_m$ be the posterior distribution computed by a probabilistic method solving \eref{Eq:Axb}, and let $\qvec$ be a sample from $\mu_m$.
  The Weak $Z$-statistic for $\xvec_*$ is 
  \begin{equation}
    \label{Eq:ZStat}
    \WeakZ(\xvec_*) = (\qvec-\xvec_0)^T\Sigmat_0^\dagger(\qvec-\xvec_0),
  \end{equation}
  where $\Sigmat_0^\dagger$ is the Moore-Penrose inverse of $\Sigmat_0$. The Weak $Z$-statistic depends on $\xvec_*$ if the posterior $\mu_m$ depends on $\xvec_*$.
  If $\xvec_*$ is drawn from $\mu_0$ and the method that produces $\mu_m$ is weakly calibrated, then the Weak $Z$-statistic is distributed according to the chi-square distribution with $\rank(\Sigmat_0)$ degrees of freedom.
\end{theorem}


